A Picture is Worth a Thousand Prompts? Efficacy of Iterative Human-Driven Prompt Refinement in Image Regeneration Tasks

With AI-generated content becoming ubiquitous across the web, social media, and other digital platforms, it is vital to examine how such content are inspired and generated. The creation of AI-generated images often involves refining the input prompt iteratively to achieve desired visual outcomes. This study focuses on the relatively underexplored concept of image regeneration using AI, in which a human operator attempts to closely recreate a specific target image by iteratively refining their prompt. Image regeneration is distinct from normal image generation, which lacks any predefined visual reference. A separate challenge lies in determining whether existing image similarity metrics (ISMs) can provide reliable, objective feedback in iterative workflows, given that we do not fully understand if subjective human judgments of similarity align with these metrics. Consequently, we must first validate their alignment with human perception before assessing their potential as a feedback mechanism in the iterative prompt refinement process. To address these research gaps, we present a structured user study evaluating how iterative prompt refinement affects the similarity of regenerated images relative to their targets, while also examining whether ISMs capture the same improvements perceived by human observers. Our findings suggest that incremental prompt adjustments substantially improve alignment, verified through both subjective evaluations and quantitative measures, underscoring the broader potential of iterative workflows to enhance generative AI content creation across various application domains.

==> exp-setup.tex <==
\section{Experimental Setup}
\label{sec:exp-setup}






























==> paperchecklist.tex <==





\subsection*{Paper Checklist}
\label{sec:checklist}

\begin{enumerate}
\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
    \answerYes{Yes, this survey should not have any of the negative impact mentioned above.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes, they do.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes, our research questions and motivation are based on prior work and literature reviews.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, refer to the ``Limitations and Future Work" section\ref{sec:limitations-futurework}.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, refer to the ``Limitations and Future Work" section\ref{sec:limitations-futurework}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Yes, refer to the ``Implications from Results" section\ref{sec:implications}.}
    \item Did you discuss any potential misuse of your work?
    \answerYes{Yes, refer to the ``Implications from Results" section\ref{sec:implications}.}
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, we discussed data collection and handling in the ``Participant Recruitment and Data Handling" section in the Appendix\ref{appendix:consent}. The dataset and survey interface code will be released to a public facing repository for reproducibility pending acceptance.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes, we have.}
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerYes{Yes, refer to the ``Research Questions and Hypotheses" and ``Experimental Setup and Evaluation" sections.}
  \item Have you provided justifications for all theoretical results?
    \answerYes{Yes, refer to refer to the ``Research Questions and Hypotheses" and ``Implications from Restuls" sections.}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerYes{Yes, refer to refer to the ``Research Questions and Hypotheses" section.}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerYes{Yes, for RQ2 in the ``Research Questions and Hypotheses" section\ref{sec:goals}; hypotheses 2.1 and 2.3 serves as an objective (ISM) and subjective (user's top ranked image) explanations.}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerYes{Yes, refer to the ``Limitations and Future Work" section\ref{sec:limitations-futurework}.}
  \item Have you related your theoretical results to the existing literature in social science?
    \answerYes{Yes, refer to the ``Experimental Setup and Evaluation" section\ref{sec:eval}.}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerYes{Yes, refer to the ``Implications from Results" section\ref{sec:implications}.}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{No, we did not. However, we will release the source code for the survey interface, the data, and setup instructions to a public facing repository and include it as an URL pending acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, refer to the ``Chosen AI-Image Generation Model" section\ref{sec:chosen-model}.}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{No, as the seed were fixed in for the generation, refer to the ``Chosen AI-Image Generation Model" section\ref{sec:chosen-model}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, refer to the ``Chosen AI-Image Generation Model" section\ref{sec:chosen-model}.}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, refer to the ``Research Questions and Hypotheses", ``Experimental Setup and Evaluation", and ``Discussion" sections.}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
    \answerNo{No, as we did not do a traditional ``machine learning" experiment so misclassification and fault (in)tolerance did not apply.}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, refer to the ``Chosen AI-Image Generation Model" section\ref{sec:chosen-model}.}
  \item Did you mention the license of the assets?
    \answerYes{Yes, refer to the ``Chosen AI-Image Generation Model" section\ref{sec:chosen-model}.}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerNA{NA}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes, refer to the ``Participant Recruitment and Data Handling" section in the Appendix\ref{appendix:consent}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Yes, refer to the ``Participant Recruitment and Data Handling" section in the Appendix\ref{appendix:consent}.}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerNo{No, we did not. However, pending acceptance, we plan on releasing the dataset on a public facing repository pending acceptance.}
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerNo{No, we did not. However, we will be releasing the dataset and appropriate Datasheet to a public facing repository pending acceptance.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects, \textbf{without compromising anonymity}...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerYes{Yes, refer to the ``Survey Instructions and Screenshots" section in the Appendix for example screenshots.}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerYes{Yes, refer to the ``Participant Recruitment and Data Handling" section in the Appendix\ref{appendix:consent}.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{Yes, refer to the ``Survey Responses Statistics" section\ref{sec:survey-stats}.}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerYes{Yes, refer to the ``Participant Recruitment and Data Handling" section in the Appendix\ref{appendix:consent}.}
\end{enumerate}

\end{enumerate}


==> rq.tex <==
RQ1: Do humans generally agree that the selected Image Similarity Metrics (ISMs) are good numeric heuristics for whether a human perceives two images as similar or different? (this is because we use these metrics for the later analysis.) To what extent do metric values correlate with user-perceived image similarity in the final ranked image set?

Hypothesis 1.1: Human raters do show high agreement with the ISMs.

Hypothesis 1.2: No significant differences in agreement between the ISMs.

Supporting Reference(s): \cite{zhang2018perceptual}

Test: For each target prompt (a set), the human ranked all their generated images for the set based on how closely they perceive their generated images are to the target image. We compare this to the relative ranking of a given ISM against the same set of generated images to the target image to calculate cohens alpha to measure intraclass correlation coefficient (ICC). Given the ICC average for each ISM, if Hypothesis 1.1 holds, the ICC average for a given ISM should be between 0.5-0.9 (Moderate to Good) CITE. If H1.2 holds, we should see all ISMs in the same range of by ICC. 

RQ2: Given the task of prompt inference to regenerate a target image, does iterative prompt inference improve the ISM of a user-generated image, meaning it is more closely aligned with the target image?

Hypothesis 2.1: Successive prompt inference will lead to an improvement in user's ISM score.

Hypothesis 2.2: The marginal improvement in ISM score will decrease with successive iterations, eventually reaching a plateau.

Supporting Reference(s):

Test: Through a mixed-effects model, take into account nested repeated measures of iteration and target prompt, fixed effects for what factors such as iteration, user demographics, and metric type, random effect for each user in the study and target prompt. Expect to see significant fixed effect for iteration, where successive iterations have higher scores until a given iteration, and past this point, successive iterations do not significantly improve ISM score (are not significant).



RQ3: Does displaying the ISM score from the previous iteration influence the improvement of users' ISMs in subsequent iterations?

Hypothesis 3: Providing users with their ISM score from the previous iteration yields a greater marginal improvement in ISM score for subsequent iterations. (The presence of metric feedback reduces the number of iterations needed to reach a plateau in ISM score/causes the improvement in ISM score to decay faster.)

Supporting Reference(s):

Test: Build a linear mixed model with same structure as RQ2 but with the interaction term `iteration*metric\_shown`. If H3 holds, then iteration will be a significant fixed effect, and the interaction term of `iteration*metric\_shown` will also be significant, and the coefficient of that interaction term will be negative. 















